A Review of AI and Machine Learning Contribution in Predictive Business Process Management (Process Enhancement and Process Improvement Approaches)

Purpose- The significance of business processes has fostered a close collaboration between academia and industry. Moreover, the business landscape has witnessed continuous transformation, closely intertwined with technological advancements. Our main goal is to offer researchers and process analysts insights into the latest developments concerning Artificial Intelligence (AI) and Machine Learning (ML) to optimize their processes in an organization and identify research gaps and future directions in the field. Design/methodology/approach- In this study, we perform a systematic review of academic literature to investigate the integration of AI/ML in business process management (BPM). We categorize the literature according to the BPM life-cycle and employ bibliometric and objective-oriented methodology, to analyze related papers. Findings- In business process management and process map, AI/ML has made significant improvements using operational data on process metrics. These developments involve two distinct stages: (1) process enhancement, which emphasizes analyzing process information and adding descriptions to process models, and (2) process improvement, which focuses on redesigning processes based on insights derived from analysis. Research limitations/implications- While this review paper serves to provide an overview of different approaches for addressing process-related challenges, it does not delve deeply into the intricacies of fine-grained technical details of each method. This work focuses on recent papers conducted between 2010 and 2024. Originality/value- This paper adopts a pioneering approach by conducting an extensive examination of the integration of AI/ML techniques across the entire process management lifecycle. Additionally, it presents groundbreaking research and introduces AI/ML-enabled integrated tools, further enhancing the insights for future research.

==> References/Literature_Reviews.tex <==
\begin{table}[htbp]
\centering
\caption{Process Improvement and Enhancement Literature}
\label{tab:process_literature}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Name & Year & Process Improvement & Process Enhancement & Methods and Approach Introduction & Terminological & Actors and Tools & Challenges and Issues & Sustainability Criteria & Case Study \\
\hline
(Zellner, 2011) & 2011 & a & a & & & & & & & General \\
(Vom Brocke and Sinnl, 2011) & 2011 & a & & & & & & & & General \\
(Seethamraju, 2012) & 2012 & a & & & & & & & & General \\
(Segatto et al., 2013) & 2013 & a & & & & & & & & General \\
(Uriona Maldonado et al., 2014) & 2014 & a & & a & & & & & & General \\
(Mendes and Bax, 2014) & 2014 & a & & a & & & & & & General \\
(Rojas et al., 2016) & 2016 & & a & a & & & & & & Healthcare \\
(Alotaibi, 2017) & 2017 & a & & & a & & a & & a & General \\
(Pourmirza et al., 2017) & 2017 & a & & & & a & & & & General \\
(Bazan and Estevez, 2017) & 2017 & a & & & & & & & & General \\
(Arias et al., 2018) & 2018 & a & & & a & & & & & General \\
(Sujová et al., 2018) & 2018 & a & & & & a & a & & & General \\
(Danilova, 2019) & 2019 & a & & & a & & & & & General \\
(Ahmad and Looy, 2020) & 2020 & a & & a & & & & & & General \\
(Vecino Sato et al., 2021) & 2021 & & a & & & & & & & General \\
(Guzzo et al., 2021) & 2021 & & a & & & & a & & a & Healthcare \\
(Marin-Castro and Tello-Leal, 2021) & 2021 & a & a & & & & & a & & General \\
(Malinova et al., 2022) & 2022 & a & & a & & & & & & General \\
(Viriyasitavat et al., 2022) & 2022 & a & & & & a & & & & General \\
This Work & 2023 & a & a & a & & & a & & a & General \\
\hline
\end{tabular}
\end{table}

==> References/Not_Necessary.tex <==
{\color{blue}The following two paragraphs can be moved to a later section, or removed completely. }

In light of the extensive body of literature that has been developed and expanded in this field, the researchers in a terminological framework, attempt to define the scope of BPM strictly in order to refrain from using other terms such as Enterprise Content Management(ECM)~\cite{Mendes2018}  and Lean Management (LM)~\cite{UrionaMaldonado2020} with BPM interchangeably.

Despite the predominant purpose of review papers being centered around economic objectives, there has been a significant shift in recent years. As sustainability has gained greater prominence in organizational priorities, considerable efforts have been made to address social issues~\cite{Bazan2020} for increasing collaboration, monitoring, participation, and knowledge management and environmental  issues~\cite{Couckuyt2020} for leading to a greater sense of responsibility toward society among organizations. 

==> Table_related_work.tex <==
\begin{table}[!ht]
\centering
\caption{Related Works}
\label{Related Works}
\resizebox{500pt}{!}{
\begin{tabular}{cccccccccccccccccc}
\hline
\multirow{2}{*}{Name}       & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Process\\ Improvement\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Process\\ Enhancement\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Methods and Approach\\ Introduction\end{tabular}} &  & \multicolumn{5}{c}{Actors and Tools}                                                                                                                                                                                                                                        &  & \multicolumn{5}{c}{Challenges and Issues}                                                                                                                                                                                                                                  & \multirow{2}{*}{Case Study} \\ \cline{4-5} \cline{7-11} \cline{13-17}
                            &                                                                                &                                                                                & Contributions                                    & Objectives                                   &  & \begin{tabular}[c]{@{}c@{}}Process \\ Owners\end{tabular} & BPMS       & \begin{tabular}[c]{@{}c@{}}Digital \\ Transforamtion\end{tabular} & \begin{tabular}[c]{@{}c@{}}Culture and \\ Team\end{tabular} & \begin{tabular}[c]{@{}c@{}}AI & \\ Machine Learning\end{tabular} &  & Agility    & \begin{tabular}[c]{@{}c@{}}Insufficient \\ Knowdelge\end{tabular} & \begin{tabular}[c]{@{}c@{}}Change \\ Management\end{tabular} & \begin{tabular}[c]{@{}c@{}}Security \\ Requirements\end{tabular} & \begin{tabular}[c]{@{}c@{}}Data\\ Cleaning\end{tabular} &                             \\ \cline{1-5} \cline{7-11} \cline{13-18} 
\citep{Zellner2011}         & \checkmark                                                                     &                                                                                & \checkmark                                       &                                              &  &                                                           &            &                                                                   &                                                             &                                                                  &  &            & \checkmark                                                        &                                                              & \multicolumn{1}{l}{}                                             & \multicolumn{1}{l}{}                                    & General                     \\
\citep{VomBrocke2011}       & \checkmark                                                                     &                                                                                &                                                  &                                              &  &                                                           &            &                                                                   & \checkmark                                                  &                                                                  &  &            &                                                                   &                                                              & \multicolumn{1}{l}{}                                             & \multicolumn{1}{l}{}                                    & General                     \\
\citep{Seethamraju2012}     & \checkmark                                                                     &                                                                                &                                                  &                                              &  &                                                           &            &                                                                   &                                                             &                                                                  &  &            &                                                                   &                                                              &                                                                  &                                                         & General                     \\
\citep{Segatto2013}         & \checkmark                                                                     &                                                                                &                                                  &                                              &  &                                                           &            &                                                                   &                                                             &                                                                  &  &            &                                                                   &                                                              &                                                                  &                                                         & General                     \\
\citep{UrionaMaldonado2020} & \checkmark                                                                     &                                                                                &                                                  &                                              &  &                                                           &            &                                                                   &                                                             &                                                                  &  &            &                                                                   &                                                              &                                                                  &                                                         & General                     \\
\citep{Mendes2018}          & \checkmark                                                                     &                                                                                &                                                  &                                              &  &                                                           &            &                                                                   &                                                             &                                                                  &  &            &                                                                   &                                                              &                                                                  &                                                         & General                     \\
\citep{rojas2016process}    &                                                                                & \checkmark                                                                     & \checkmark                                       & \checkmark                                   &  &                                                           &            &                                                                   &                                                             &                                                                  &  &            &                                                                   &                                                              &                                                                  &                                                         & Healthcare                  \\
\citep{Alotaibi2017}        & \checkmark                                                                     &                                                                                &                                                  &                                              &  &                                                           &            &                                                                   &                                                             &                                                                  &  & \checkmark & \checkmark                                                        &                                                              & \checkmark                                                       &                                                         & General                     \\
\citep{Pourmirza2017}       & \checkmark                                                                     &                                                                                &                                                  &                                              &  &                                                           & \checkmark &                                                                   &                                                             &                                                                  &  &            &                                                                   &                                                              &                                                                  &                                                         & General                     \\
\citep{Bazan2020}           & \checkmark                                                                     &                                                                                &                                                  &                                              &  &                                                           &            &                                                                   &                                                             &                                                                  &  &            &                                                                   &                                                              &                                                                  &                                                         & General                     \\
\citep{Arias2018}           & \checkmark                                                                     &                                                                                &                                                  &                                              &  &                                                           &            &                                                                   & \checkmark                                                  &                                                                  &  &            &                                                                   &                                                              &                                                                  &                                                         & General                     \\
\citep{Sujova2018}          & \checkmark                                                                     &                                                                                &                                                  &                                              &  &                                                           &            &                                                                   &                                                             &                                                                  &  &            & \checkmark                                                        & \checkmark                                                   &                                                                  &                                                         & General                     \\
\citep{Danilova2019}        & \checkmark                                                                     &                                                                                &                                                  &                                              &  & \checkmark                                                &            &                                                                   & \checkmark                                                  &                                                                  &  &            &                                                                   &                                                              &                                                                  &                                                         & General                     \\
\citep{Ahmad2020}           & \checkmark                                                                     &                                                                                &                                                  & \checkmark                                   &  &                                                           &            & \checkmark                                                        &                                                             &                                                                  &  &            &                                                                   &                                                              &                                                                  &                                                         & General                     \\
\citep{sato2021survey}      &                                                                                & \checkmark                                                                     &                                                  &                                              &  &                                                           &            &                                                                   &                                                             &                                                                  &  &            &                                                                   &                                                              &                                                                  &                                                         & General                     \\
\citep{guzzo2022process}    &                                                                                & \checkmark                                                                     &                                                  &                                              &  &                                                           &            &                                                                   &                                                             &                                                                  &  &            &                                                                   &                                                              &                                                                  &                                                         & Healthcare                  \\
\citep{marin2021event}      &                                                                                & \checkmark                                                                     & \checkmark                                       &                                              &  &                                                           &            &                                                                   &                                                             &                                                                  &  &            &                                                                   &                                                              &                                                                  & \checkmark                                              & General                     \\
\citep{Malinova2022}        & \checkmark                                                                     &                                                                                & \checkmark                                       & \checkmark                                   &  &                                                           &            &                                                                   &                                                             &                                                                  &  &            &                                                                   &                                                              &                                                                  &                                                         & General                     \\
\citep{Viriyasitavat2022}   & \checkmark                                                                     &                                                                                &                                                  &                                              &  &                                                           &            & \checkmark                                                        &                                                             &                                                                  &  &            &                                                                   &                                                              &                                                                  &                                                         & General                     \\
This Work                   & \checkmark                                                                     & \checkmark                                                                     & \checkmark                                       & \checkmark                                   &  &                                                           &            &                                                                   & \checkmark                                                  & \checkmark                                                       &  &            &                                                                   & \checkmark                                                   &                                                                  & \checkmark                                              & General                     \\ \hline
\end{tabular}
}
\end{table}
